Evaluating FPGA Accelerator Performance with a Parameterized OpenCL Adaptation of the HPCChallenge Benchmark Suite

FPGAs have found increasing adoption in data center applications since a new generation of high-level tools have become available which noticeably reduce development time for FPGA accelerators and still provide high quality of results. There is however no high-level benchmark suite available which specifically enables a comparison of FPGA architectures, programming tools and libraries for HPC applications. To fill this gap, we have developed an OpenCL-based open source implementation of the HPCC benchmark suite for Xilinx and Intel FPGAs. This benchmark can serve to analyze the current capabilities of FPGA devices, cards and development tool flows, track progress over time and point out specific difficulties for FPGA acceleration in the HPC domain. Additionally, the benchmark documents proven performance optimization patterns. We will continue optimizing and porting the benchmark for new generations of FPGAs and design tools and encourage active participation to create a valuable tool for the community.

==> global_memory_bandwidth.tex <==


\todo{Move STREAM and RA results here, add Xilinx results and discuss separately. Remaining benchmarks in separate section. This should make it less competitive. Just discuss measured and expected performance}


==> models.tex <==

\subsection{STREAM}

The STREAM benchmark consists of four different vector operations on three arrays.
The \emph{copy} and \emph{scale} kernels use
one array as input and another array as output whereas the \emph{add} and \emph{triad} kernels use two arrays as input and also one as output.

All four vector operations are implemented in a single kernel.
This reduces the overall resource usage.
The kernel also contains a local memory buffer to store intermediate data before writing in back to memory.
In consequence it is possible to use a single memory bank per kernel and also reduce the interference of read and write accesses by storing the data in local memory.

For Stratix 10 the width of the memory interface is \SI{64}{\byte}. One LSU with \SI{64}{\byte} width loads a data chunk from memory. An operation is executed on the data chunk and it is written back to memory. Since these operations can be easily pipelined it can be assumed that there is one read and one write operation per cycle for large enough data arrays.
This results in the following model for the achievable data rate in \si{\byte} for a given maximum frequency $f_{max}$ of the bitstream and number of used arrays $n$:

$$ data\_rate = n * \SI{64}{\byte} * f_{max} $$

Moreover the data transfer is limited by the total bandwidth of the external memory.

$$ max\_data\_rate = n * min(\SI{64}{\byte} * f_{max}, mem_{max}) $$

where $n$ is the number of memory banks on a system.
On Stratix 10 there are four memory banks with a maximum bandwidth $mem_{max}$ of \SI{19.2}{\giga\byte} each. 
Also the maximum bandwidth of a memory bank can be fully utilized with and $f_{max}$ of \SI{300}{\mega\hertz} and above. So there is only a very small benefit for frequencies above this threshold.

$  $


==> models_old.tex <==
\begin{itemize}
    \item Introduce OpenCL for FPGA and what has to be 
    done to get performance with a kernel.
    \item Describe design of benchmark kernels and model its performance.
\end{itemize}

\subsection{STREAM}
The STREAM benchmark consists of four different kernels that are implementing vector operations on three arrays.
The \emph{copy} and \emph{scale} kernels use
one array as input and another array as output whereas the \emph{add} and \emph{triad} kernels use two arrays as input and also one as output.

All kernels have a low computational intensity since they are using every value just once.
The computation will most likely be memory bound.
In consequence, only the read and write from and to global memory is considered for the performance model.

For Stratix 10 the width of the memory interface is \SI{64}{\byte}. One LSU with \SI{64}{\byte} width loads a data chunk from memory. An operation is executed on the data chunk and it is written back to memory. Since these operations can be easily pipelined it can be assumed that there is one read and one write operation per cycle for large enough data arrays.
This results in the following model for the achievable data rate in \si{\byte} for a given maximum frequency $f_{max}$ of the bitstream and number of used arrays $n$:
$$ data\_rate = n * \SI{64}{\byte} * f_{max} $$

Moreover the data transfer is of course limited by the total bandwidth of the external memory.
So the maximum achievable data rate must be the minimum of the theoretical total memory bandwidth $mem_{max}$ and the data rate calculated previously:

$$ max\_data\_rate = min(n * \SI{64}{\byte} * f_{max}, mem_{max}) $$

On Stratix 10 there are four memory banks with a maximum bandwidth of \SI{19.2}{\giga\byte} each. 
This will also limit $n$ since more arrays than memory interfaces will lead to loads and stores competing for the memory and thus a decrease of the overall bandwidth.
In the following equation the decrease is not modelled but the bandwidth is limited by the number of available memory interfaces $i$.
Also the maximum bandwidth of a memory bank can be fully utilized with and $f_{max}$ of \SI{300}{\mega\hertz} and above. So there is no benefit for frequencies above this threshold.
\todo{somewhere the Avalon MMI has to be explained: bursts are destroyed, which leads to a reduced bandwidth}

$$ max\_d = min(min(n,i) * \SI{64}{\byte} * min(f_{max},\SI{300}{\mega\hertz}), mem_{max}) $$

Where is gap between measurements and model coming from?
Measurements still increase above \SI{300}{\mega\hertz} although this should not be the case.


\todo{In another section interleaving and its impact has to be discussed}

\subsection{Random Access}

The random access benchmark randomly updates data items in an array of size $d$, which should be up to half of the available main memory.
The kernel of the benchmark implementation is replicated for all available memory banks $n$ and only in charge of updating
values in this bank.
Every kernel is calculating all $4 * d$ addresses and check if they are located in the memory bank the kernel is assigned to.
It is assumed, that the addresses are generated uniformly distributed over the range of valid addresses.
So on average every $n$-th address needs to be updated by each kernel.

The kernel contains three pipelines.
In Figure~\ref{fig:random_access} a schematic overview of the kernel is given.
The first pipeline calculates a new set of addresses from a pseudo random number scheme.
The second pipeline loads the data in these addresses from global memory if necessary.
The third pipeline updates the data and writes it back to global memory.
The pipelines use a local memory buffer $buf_{local}$ to forward the data between each other.
The buffer also specifies the depth of the pipelines together with the unrolling factor $u$.
This enables checking multiple addresses at once.
All three smaller pipelines are used in a bigger pipeline over the total number of required updates $4 * d$.

\begin{figure}
    \centering
\begin{tikzpicture}[node distance=1.5cm,
    every node/.style={fill=white, font=\sffamily}, align=center]
  % Specification of nodes (position, etc.)
  \node (calc)             [base]              {Calculate $u$ addresses\\ $\frac{buf_{local}}{u}$ times};
  \node (load)     [base, below of=calc]          {Load data \\$\frac{buf_{local}}{u}$ times};
  \node (store)      [base, below of=load]   {Store data\\ $\frac{buf_{local}}{u}$ times};
   
  % Specification of lines between nodes specified above
  % with aditional nodes for description 
  \draw[->]             (calc) -- (load);
  \draw[->]     (load) -- (store);
  \draw[->]      (store.west) -- ++(-1.5,0) -- ++(0,1.5) -- node {Repeat\\ $\frac{4 * d}{buf_{local}}$\\ times}  ++(0,1.5) -- (calc.west);

  \end{tikzpicture}
    \caption{Schematic view of the random access kernel.}
    \label{fig:random_access}
\end{figure}

For a large enough $d$ and thus a large enough total runtime the outer loop can be neglected for the target metric $GU/s$.
Thus the model is focusing on the inner loops.
Since they are also pipelined with an II of 1, the main bottleneck will be the global memory access.
First we calculate how many clock cycles will be necessary on average to process $buf_{local}$ addresses with regards to global memory latency.

$l_i = \frac{updates * 2 * 240 + i}{i}$

with $i = \frac{buf_{local}}{u}$ being the number of iterations in the inner pipelines,
$updates = \frac{u}{n}$ the number of updates that will be executed on average for $u$ addresses.
$l_i$ being the latency for one pipeline iteration.
To update a value we need to read and write to global memory once -- so we have two memory accesses per update.
The latency of such a update is 240 clock cycles taken from the report.
\todo{Check: 240 must be defined for a reference clock frequency... which one? Maybe 480MHz?}
Since everything is pipelined we assume load and store are executed in parallel and the update latency can be neglected.
The whole pipeline has an II of 1, so we will need $i$ additional clock cycles to update all $buf_{local}$ addresses.
To get the average over all iterations we have to divide by $i$.

So in $l_i$ clock cycles the kernel will update in average $\frac{u}{n} * n$ values, since the kernel is running in parallel for every memory bank.
The get the average clock cycles to update a single address can then be calculated with:
$u_i = \frac{l_i}{\frac{u}{n} * n}$

To get the final result we now need to calculate how many updates fit into a second:

$GU/s = \frac{f_{max}}{u_i} * 1.0^{-9}$

So the model takes into account the following parameters: The maximum kernel frequency $f_{max}$,
the number of global memory banks $n$, the size of the local memory buffer $buf_{local}$ and the
unrolling factor of the inner loops $u$.

\subsection{Matrix Transposition}

The matrix transposition benchmark calculates the following:

$C = A^T + B$

where $A$, $B$, $C$ are quadratic matrices of the same size.
The kernel is implemented as a blocked algorithm consisting of two pipelines.
In the \emph{read pipeline} a block $a_{i,j}$ of $A$ is loaded from global memory to local memory.
The block will be transposed while reading and writing to local memory.
In the \emph{write pipeline} the block $b_{j,i}$ of matrix $B$ will be loaded from global memory and $C$
will be updated with $c_{j,i} = a_{i,j}^T + b_{j,i}$.

The expected bottleneck of this algorithm is the streamed transposition of $A$, since it has to be written and read from
local memory. 

In the \emph{read pipeline} $\frac{\SI{512}{\bit}}{\SI{32}{\bit}} = 16$ floating point values of $A$ will be read from global memory per clock cycle.
In the \emph{write pipeline} the local memory is blocked by the previously loaded values and thus the \emph{read pipeline} will stall.

For the performance model we calculate the total number of clock cycles needed for quadratic matrices of size $n$.

$cycles = (\frac{n^2}{unroll} + \frac{n}{b}^2 * mem\_delay ) * 2$

with $unroll$ being the used unrolling factor, $b$ the used block size and $mem\_delay$ the delay in clock cycles to access a value from global memory.

A simpler model that assumes a fully pipelined approach without stalls would result in 

$cycles = (\frac{n^2}{unroll} + mem_delay$

For Stratix 10 the memory delay is assumed to be 240 and 16 is used as the unrolling factor.
As already mentioned we use a streaming approach for the kernel, so the expected bottleneck will be the global memory.
In the \emph{read pipeline} $A$ will be loaded and in the \emph{write pipeline} $B$ will be loaded and $C$ will be stored.
So we need $\frac{n^2}{unroll} * 2$ load operations. 
Writing $C$ can be neglected since we do it at the same time than loading $B$.
Moreover we have to consider pipeline delays.
The pipelines have to be started for every block of the matrix $\frac{n}{b}^2$ and will need $mem\_delay$ clock cycles to retrieve the first values from global memory.
After that they will get $unroll$ values from memory every clock cycle.

The execution time can than be calculated:

$t_{exe} = \frac{cycles}{f_{max}}$

where $f_{max}$ is the maximum frequency of the kernel.

\subsection{GEMM}

The kernel of the benchmark calculates the following:

$C_{out} = \alpha * C + \beta * A * B$

where $A$, $B$, $C$ and $C_{out}$ are quadratic matrices and $\alpha$ and $\beta$ scalar values.
The kernel follows a three-leveled approach.
On the first level we calculate $A*B$ in a blocked algorithm.
The second level calculates the result for a block of $A*B$ also in a blocked fashion in local memory.
The third level calculates on even smaller blocks in registers using the cannon algorithm.

\todo{Finish the model for GEMM}

\subsection{Effective Bandwidth Benchmark}

The $b_{eff}$ benchmark targets the network of a system.
In case of the FPGAs it will benchmark the performance of the external channels by producing a metric
that is called the \emph{effective bandwidth}. 
It is an accumulation of achieved bandwidths in the network for different message sizes and communication patterns and is given in \si{\giga\byte\per\second}.
Since the \acp{FPGA} are using a \ac{CSN} without an additional layer it is sufficient to use a single communication pattern.
So the effective bandwidth will be calculated with:

$b_{eff} = \frac{\sum_L b_L}{21}$

with $b_L$ being the achieved bandwidth with message size $L$.
The bandwidth will be measured for 21 different message sizes and so the sum has to be divided by 21.
The duration of a message exchange will be measured and used to calculate the bandwidth.
The exchange will be repeated multiple times to reduce measurement errors caused by short runtimes.

For the measurement two \acp{FPGA} are used that will execute two kernels:

\begin{itemize}
    \item \emph{send}: This kernel will first send and then receive a message over the external channel in a loop.
    \item \emph{recv}: This kernel will first receive and then send a message over the external channel in a loop.
\end{itemize}

The \emph{send} kernel of the first \ac{FPGA} will be connected to the \emph{recv} kernel of the second \ac{FPGA} over the external channels and the other way around.
Since there might be more than two external channels available on the board the kernels can also use multiple channels for communication.

The achievable bandwidth for the communication between a \emph{send} and \emph{recv} kernel can be calulated with:

$b_{L} = \frac{L}{\frac{ceil(\frac{L}{c * c_{width}})}{c_{frequency}} + c_{latency}}$

where $ceil(\frac{L}{c * c_{width}})$ is the number of clock cycles needed to send the message over the given channels. $L$ is the message size, $c$ the number of channels and $c_{width}$ the width of a single channel. 
This has to be divided by the channel clock frequency $c_{frequency}$ to get the time necessary to send the message. 
The channel latency $c_latency$ has to be added to this time since we do a message exchange and the \emph{recv} kernel will only start sending its own message after it received the message.

Combining this model with the calculation of $b_{eff}$ we can expect an effective bandwidth of \SI{4.09}{\giga\byte\per\second} per \emph{send} and \emph{recv} pair.
This value can be used to calculate the effective bandwidth for different ring sizes by just multiplying the value according to the number of kernel pairs used.

